Optimization-Based Outlier Accommodation for Tightly Coupled RTK-Aided Inertial Navigation Systems in Urban Environments

Global Navigation Satellite Systems (GNSS) aided Inertial Navigation System (INS) is a fundamental approach for attaining continuously available absolute vehicle position and full state estimates at high bandwidth. For transportation applications, stated accuracy specifications must be achieved, unless the navigation system can detect when it is violated. In urban environments, GNSS measurements are susceptible to outliers, which motivates the important problem of accommodating outliers while either achieving a performance specification or communicating that it is not feasible. Risk-Averse Performance-Specified (RAPS) is designed to optimally select measurements to address this problem. Existing RAPS approaches lack a method applicable to carrier phase measurements, which have the benefit of measurement errors at the centimeter level along with the challenge of being biased by integer ambiguities. This paper proposes a RAPS framework that combines Real-time Kinematic (RTK) in a tightly coupled INS for urban navigation applications. Experimental results demonstrate the effectiveness of this RAPS-INS-RTK framework, achieving 85.84% and 92.07% of horizontal and vertical errors less than 1.5 meters and 3 meters, respectively, using a smartphone-grade Inertial Measurement Unit (IMU) from a deep-urban dataset. This performance not only surpasses the Society of Automotive Engineers (SAE) requirements, but also shows a 10% improvement compared to traditional methods.

==> Sections/raps.tex <==
\subsection{GNSS Measurements}
GNSS measurements are used to estimate the absolute positions. This paper focus on \ac{DGNSS}. After compensating for the common-mode errors through single-difference (between receivers) operation, the linearized double-difference (between satellites $s$ and pivot satellite $o$) pseudorange and phase measurements for satellite $s$ is modeled as
\begin{align}
	\delta \rho_{s,o} = \delta\1_s^r 
\end{align}


The paper only uses single differenced GNSS measurements. The single differenced GNSS pseudorange measurement model at time $k$ for satellite $s$ is
\begin{equation}
	\Delta \rho_{s,k} = R(p_k, \hat{p}_{s,k}) + c_{b,k} + M_{p,k}^s + \eta_{s,k}
\end{equation}
where $R(p_k, \hat{p}_{s,k}) = |p_k - \hat{p}_{s,k}|$, $c_b$ is the receiver clock bias, $M_p^s$ is multipath error, and $\eta_{s,k} \sim \mathcal{N}(0, R_p)$ is receiver pseudorange noise. The Doppler $D_{s,r}$ measurement model is:
\begin{equation}
	\lambda D_{s,k} = h_{s,k} v_k + c_{d,k} + \epsilon_{s,k}
\end{equation}
where $h_{s,k} = \frac{p_k - \hat{p}_{s,k}}{|p_k - \hat{p}_{s,k}|}$ is the line-of-sight vector from receiver to satellite $s$, $v$ is the rover velocity vector, and $\epsilon_{s,k} \sim \mathcal{N}(0, R_d)$ is Doppler measurement noise.

Denote the measurement vector for satellite $s$ at time $k$ as $\mathbf{z}_{s,k} = [\Delta \rho_{s,k}, \lambda D_{s,k}]^\top$ which is modeled as
\begin{equation}
	\mathbf{z}_{s,k} = h(\mathbf{x}_k) + \gamma_{s,r,k},
\end{equation}
where the function $h(\mathbf{x}_k)$ is
\begin{equation}
	h(\mathbf{x}_k) = \begin{bmatrix} R(p_k, \hat{p}_{s,k}) + c_{b,k} + M_{p,k}^s \\ h_{s,k} v_k + c_{d,k} \end{bmatrix},
\end{equation}
and $\gamma_{s,r,k} = \begin{bmatrix} \eta_{s,k} \\ \epsilon_{s,k} \end{bmatrix} \sim \mathcal{N}(0, R)$ with $R = \begin{bmatrix} R_p & 0 \\ 0 & R_d \end{bmatrix}$.

The predicted measurement and measurement residual are computed as
\begin{equation}
	\hat{\mathbf{z}}_{s,k} = h(\hat{\mathbf{x}}_{k}^-) \text{ and } \delta \mathbf{z}_{s,k} = \mathbf{z}_{s,k} - \hat{\mathbf{z}}_{s,k},
\end{equation}
with linearized residual modeled as
\begin{equation}
	\delta \mathbf{z}_{s,k} = \mathbf{H}_{s,k} \delta \mathbf{x}_k + \gamma_{s,r,k}
\end{equation}
with $\delta \mathbf{x}_k = \mathbf{x}_k - \hat{\mathbf{x}}_k$, and measurement matrix $\mathbf{H}_{s,k} = \begin{bmatrix} \mathbf{h}_{s,k} & 0 & 0 & 0 & 0 & 1 & 0 & \mathbf{e}_s \\ 0 & \mathbf{h}_{s,k} & 0 & 0 & 0 & 0 & 1 & 0 \end{bmatrix}$,
where the boldface symbols in the last column are $m$ element row vectors, with $\mathbf{e}_s$ being row $s$ of the identity matrix. The concatenation of the residuals per satellite will be denoted by
\begin{equation}
	\mathbf{r}_k = \mathbf{H}_k \delta \mathbf{x}_k + \gamma_k
\end{equation}
where $\mathbf{H}_k$ and $\gamma_k$ are the concatenation of $\mathbf{H}_{s,k}$ and $\gamma_{s,r,k}$, respectively.
